Deep Understanding of Sign Language for Sign to Subtitle Alignment

The objective of this work is to align asynchronous subtitles in sign language videos with limited labelled data. To achieve this goal, we propose a novel framework with the following contributions: (1) we leverage fundamental grammatical rules of British Sign Language (BSL) to pre-process the input subtitles, (2) we design a selective alignment loss to optimise the model for predicting the temporal location of signs only when the queried sign actually occurs in a scene, and (3) we conduct self-training with refined pseudo-labels which are more accurate than the heuristic audio-aligned labels. From this, our model not only better understands the correlation between the text and the signs, but also holds potential for application in the translation of sign languages, particularly in scenarios where manual labelling of large-scale sign data is impractical or challenging. Extensive experimental results demonstrate that our approach achieves state-of-the-art results, surpassing previous baselines by substantial margins in terms of both frame-level accuracy and F1-score. This highlights the effectiveness and practicality of our framework in advancing the field of sign language video alignment and translation.

==> tab/ablation_pre.tex <==

\begin{table}[t!]
  \renewcommand{\arraystretch}{1.2}
  \renewcommand{\tabcolsep}{1.2mm}
  \centering
  \caption{Ablation study on subtitle pre-processing.}
  \resizebox{0.999\linewidth}{!}{
  \begin{tabular}{l|cccc}
    \toprule
    Method & frame-acc ($\%$) $\uparrow$ & F1@.10 $\uparrow$ & F1@.25 $\uparrow$ & F1@.50 $\uparrow$ \\
    \midrule
    Baseline with SA loss & 73.77 & 76.93 & 69.95 & 57.36 \\
    % + stopwords & 75.15 & 79.35 & 72.65 & 60.05 \\
    % + remove punctuation & 74.12 & 77.85 & 71.00 & 58.51 \\
    % + fix contractions & 75.23 & 79.57 & 73.02 & 60.72 \\
    + stopwords & 75.23 & 79.57 & 73.02 & 60.72 \\
    ~+ remove articles & 75.43 & 79.72 & 73.45 & 60.85 \\
    ~~+ lemmatise & 75.46 & 79.88 & 73.48 & 61.21 \\
    % + remove be & 74.86 & 79.41 & 72.60 & 59.80 \\
    % + replace with been & 75.10 & 79.21 & 72.60 & 60.28 \\
    ~~~+ `be' verb process \textbf{(Ours)} & 75.64 & 80.02 & 73.35 & 61.45 \\
    \bottomrule
  \end{tabular}}
  \label{tab:textpreprocess}
\end{table}

==> tab/inference_speed.tex <==
\begin{table}
  \centering
  \caption{Inference speed comparison.}  \resizebox{0.45\linewidth}{!}{
  \begin{tabular}{l|c}
    \toprule
    Method & time (sec) $\downarrow$ \\
    \midrule
    Text2Gloss~\cite{gomez2021syntax} & 10307.8 \\
    Ours & 8.5 \\
    \bottomrule
  \end{tabular}}
  \label{tab:speed}
\end{table}

==> tab/span.tex <==
\begin{table}[!t]
  \renewcommand{\arraystretch}{1.2}
  \renewcommand{\tabcolsep}{2mm}
  \centering
  \caption{Analysis of frame-level accuracy based on ground truth span length. The higher, the better.}  \resizebox{0.95\linewidth}{!}{
  \begin{tabular}{lc|cccccc}
    \toprule
    \multirow{2}{*}{Method} & \multirow{3.15}{*}{All} & \multicolumn{6}{c}{Span Length (s)} \\
    &&0-2 & 2-4 & 4-6 & 6-8 & 8-10 & $>$ 10 \\
    % & 100$\%$ & 32.3$\%$ & 26.2$\%$ & 16.3$\%$ & 10.6$\%$ & 6.9$\%$ & 7.7$\%$ \\
    \midrule
    $S^+_{audio}$ & 85.39 & 90.73 & 85.50 & 83.04 & 81.41 & 79.90 & 77.98 \\
    SAT & 89.15 & 93.47 & 89.08 & 87.00 & 86.28 & 85.16 & 83.33 \\
    Ours & 91.21 & 94.10 & 91.27 & 90.05 & 89.60 & 88.29 & 86.15 \\
    \bottomrule
  \end{tabular}}
  \label{tab:spanlength}
\end{table}

==> tab/threshold.tex <==
\begin{table}
  \renewcommand{\arraystretch}{1}
  \renewcommand{\tabcolsep}{1.1mm}
  \centering
  \caption{Ablation study on the threshold.}
  \resizebox{0.95\linewidth}{!}{
  \begin{tabular}{l|cccc}
    \toprule
    Threshold & frame-acc ($\%$) $\uparrow$ & F1@.10 $\uparrow$ & F1@.25 $\uparrow$ & F1@.50 $\uparrow$ \\
    \midrule
    0.1 & 78.42 & \bf{83.30} & \bf{77.25} & 64.94 \\
    0.2 & \bf{78.70} & 83.00 & 76.97 & \bf{65.00} \\
    0.3 & 78.19 & 82.32 & 76.09 & 64.74 \\
    0.4 (Ours) & 77.22 & 81.39 & 75.03 & 63.81 \\
    0.5 & 75.71 & 79.75 & 73.51 & 62.42 \\
    0.6 & 73.58 & 77.75 & 71.20 & 59.77 \\
    0.7 & 70.45 & 74.41 & 67.85 & 56.13 \\
    0.8 & 65.56 & 68.88 & 62.41 & 50.07 \\
    0.9 & 56.31 & 57.63 & 51.25 & 37.34 \\
    \bottomrule
  \end{tabular}}
  \label{tab:tau}
\end{table}
